A Full-Stack Open-Source Framework for Antenna and Beamforming Evaluation in mmWave 5G NR

Millimeter wave (mmWave) communication represents one of the main innovations of the next generation of wireless technologies, allowing users to reach unprecedented data rates. To overcome the high path loss at mmWave frequencies, these systems make use of directional antennas able to focus the transmit power into narrow beams using BeamForming (BF) techniques, thus making the communication directional. This new paradigm opens up a set of challenges for the design of efficient wireless systems, in which antenna and BF components play an important role also at the higher layer of the protocol stack. For this reason, accurate modeling of these components in a full-stack simulation is of primary importance to understand the overall system behavior. This paper proposes a novel framework for the end-to-end simulation of 5G mmWave cellular networks, including a ray-tracing based channel model and accurate models for antenna arrays and BF schemes. We showcase this framework by evaluating the performance of different antenna and BF configurations considering both link-level and end-to-end metrics and present the obtained results.

==> figures/antenna-comparison/snr-sinr/cdf_sinr_enb8x8_ue4x4_bfTypeMmWaveCodebookBeamforming_cbUpdatePeriod100.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={SINR [dB]},
xmajorgrids,
xmin=-65.71438, xmax=79.85038,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-0.0499226690234202, ymax=1.04999631757254,
ytick style={color=black},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [semithick, color0]
table {%
-57.3563 7.36485491235823e-05
-56.0830383838384 7.36485491235823e-05
-54.8097767676768 7.36485491235823e-05
-53.5365151515151 0.000220945647370747
-52.2632535353535 0.000368242745617911
-50.9899919191919 0.000441891294741494
-49.7167303030303 0.000441891294741494
-48.4434686868687 0.000515539843865076
-47.1702070707071 0.000736485491235823
-45.8969454545455 0.000957431138606569
-44.6236838383838 0.00132567388422448
-43.3504222222222 0.00147297098247165
-42.0771606060606 0.00169391662984239
-40.803898989899 0.00198851082633672
-39.5306373737374 0.00220945647370747
-38.2573757575758 0.00272499631757254
-36.9841141414141 0.00368242745617911
-35.7108525252525 0.00390337310354986
-34.4375909090909 0.0045662100456621
-33.1643292929293 0.00530269553689792
-31.8910676767677 0.00626012667550449
-30.6178060606061 0.00751215201060539
-29.3445444444444 0.00891147444395345
-28.0712828282828 0.0104580939755487
-26.7980212121212 0.0117837678597732
-25.5247595959596 0.013404035940492
-24.251497979798 0.0147297098247165
-22.9782363636364 0.0161290322580645
-21.7049747474747 0.0178965974370305
-20.4317131313131 0.0196641626159965
-19.1584515151515 0.0219472676388275
-17.8851898989899 0.0243776697599057
-16.6119282828283 0.0279128001178377
-15.3386666666667 0.0318898217705111
-14.065405050505 0.035793194874061
-12.7921434343434 0.0399175136249816
-11.5188818181818 0.0446310207688909
-10.2456202020202 0.0513330387391368
-8.97235858585859 0.0584032994550007
-7.69909696969697 0.0670201797024599
-6.42583535353535 0.0733539549270879
-5.15257373737374 0.0807924583885697
-3.87931212121212 0.0908086610693769
-2.6060505050505 0.0986154072764766
-1.33278888888889 0.10752688172043
-0.0595272727272729 0.118353218441597
1.21373434343435 0.126970098689056
2.48699595959596 0.13404035940492
3.76025757575758 0.14287818529975
5.0335191919192 0.151126822801591
6.30678080808081 0.161953159522757
7.58004242424243 0.173221387538665
8.85330404040405 0.185226101045809
10.1265656565657 0.198777434084549
11.3998272727273 0.218367948151421
12.6730888888889 0.254897628516718
13.9463505050505 0.289512446604802
15.2196121212121 0.319782000294594
16.4928737373737 0.344380615701871
17.7661353535354 0.369494770953012
19.039396969697 0.395713654441008
20.3126585858586 0.419796730004419
21.5859202020202 0.44387980556783
22.8591818181818 0.469288555015466
24.1324434343434 0.499042568861393
25.4057050505051 0.555899248784799
26.6789666666667 0.615554573574901
27.9522282828283 0.664899101487701
29.2254898989899 0.703196347031963
30.4987515151515 0.738474002062159
31.7720131313131 0.768964501399322
33.0452747474747 0.787155693032847
34.3185363636364 0.800707026071586
35.591797979798 0.814921196052438
36.8650595959596 0.828840771836795
38.1383212121212 0.842244807777287
39.4115828282828 0.852481956105465
40.6848444444444 0.861540727647665
41.9581060606061 0.869421122403889
43.2313676767677 0.875386654882899
44.5046292929293 0.882456915598763
45.7778909090909 0.894903520400648
47.0511525252525 0.908381204890264
48.3244141414141 0.927087936367654
49.5976757575758 0.93791427308882
50.8709373737374 0.943806157018707
52.144198989899 0.947709530122257
53.4174606060606 0.952054794520548
54.6907222222222 0.956547356017087
55.9639838383838 0.964648696420681
57.2372454545455 0.975401384592724
58.5105070707071 0.980630431580498
59.7837686868687 0.982618942406835
61.0570303030303 0.983797319192812
62.3302919191919 0.986080424215643
63.6035535353535 0.990572985712181
64.8768151515152 0.993813521873619
66.1500767676768 0.994991898659596
67.4233383838384 0.997643246428045
68.6966 1
};
\addplot [semithick, color1]
table {%
-58.4492 7.36485491235823e-05
-57.1190686868687 7.36485491235823e-05
-55.7889373737374 7.36485491235823e-05
-54.4588060606061 7.36485491235823e-05
-53.1286747474747 0.000147297098247165
-51.7985434343434 0.000147297098247165
-50.4684121212121 0.000220945647370747
-49.1382808080808 0.000220945647370747
-47.8081494949495 0.000220945647370747
-46.4780181818182 0.000294594196494329
-45.1478868686869 0.000294594196494329
-43.8177555555556 0.000368242745617911
-42.4876242424242 0.000368242745617911
-41.1574929292929 0.000515539843865076
-39.8273616161616 0.000810134040359405
-38.4972303030303 0.00110472823685373
-37.167098989899 0.0012520253351009
-35.8369676767677 0.00147297098247165
-34.5068363636364 0.00176756517896597
-33.176705050505 0.00213580792458389
-31.8465737373737 0.00272499631757254
-30.5164424242424 0.0033141847105612
-29.1863111111111 0.00382972455442628
-27.8561797979798 0.00419796730004419
-26.5260484848485 0.00508174988952718
-25.1959171717172 0.00537634408602151
-23.8657858585859 0.00626012667550449
-22.5356545454545 0.00699661216674032
-21.2055232323232 0.00780674620709972
-19.8753919191919 0.0091324200913242
-18.5452606060606 0.0104580939755487
-17.2151292929293 0.0120047135071439
-15.884997979798 0.0140668728826042
-14.5548666666667 0.0170128148475475
-13.2247353535354 0.0195168655177493
-11.894604040404 0.0234202386212992
-10.5644727272727 0.0279864486669613
-9.23434141414141 0.033141847105612
-7.9042101010101 0.0399175136249816
-6.57407878787879 0.0470614228899691
-5.24394747474748 0.0561938429812933
-3.91381616161616 0.0668728826042127
-2.58368484848485 0.0786566504639859
-1.25355353535354 0.0884519074974223
0.0765777777777785 0.100898512299308
1.40670909090909 0.115701870673148
2.7368404040404 0.128516718220651
4.06697171717172 0.143688319340109
5.39710303030303 0.158344380615702
6.72723434343434 0.172926793342171
8.05736565656566 0.186330829282663
9.38749696969696 0.19921932537929
10.7176282828283 0.210413904846075
12.0477595959596 0.223007806746207
13.3778909090909 0.234202386212992
14.7080222222222 0.248416556193843
16.0381535353535 0.262483429076447
17.3682848484848 0.289217852408308
18.6984161616162 0.319045514803358
20.0285474747475 0.354102224186184
21.3586787878788 0.389011636470762
22.6888101010101 0.423847400206216
24.0189414141414 0.455442627780233
25.3490727272727 0.490867579908676
26.679204040404 0.537339814405656
28.0093353535354 0.61246133451171
29.3394666666667 0.678008543231698
30.669597979798 0.728678745028723
31.9997292929293 0.776844896155546
33.3298606060606 0.820592134334954
34.6599919191919 0.852408307556341
35.9901232323232 0.867432611577552
37.3202545454545 0.876712328767123
38.6503858585859 0.884592723523347
39.9805171717172 0.891221092944469
41.3106484848485 0.897186625423479
42.6407797979798 0.900353513035793
43.9709111111111 0.903667697746354
45.3010424242424 0.905287965827073
46.6311737373737 0.907055531006039
47.961305050505 0.910590661363971
49.2914363636364 0.919354838709677
50.6215676767677 0.926940639269406
51.951698989899 0.930770363823833
53.2818303030303 0.933716305788776
54.6119616161616 0.936588599204596
55.9420929292929 0.940197378111651
57.2722242424242 0.944984533804684
58.6023555555556 0.953159522757402
59.9324868686869 0.961334511710119
61.2626181818182 0.966268964501399
62.5927494949495 0.968625718073354
63.9228808080808 0.970098689055826
65.2530121212121 0.970761525997938
66.5831434343434 0.971939902783915
67.9132747474747 0.975254087494476
69.243406060606 0.980998674326116
70.5735373737374 0.990278391515687
71.9036686868687 0.996022978347327
73.2338 1
};
% \addplot [semithick, color2]
% table {%
% -59.0978 7.36485491235823e-05
% -57.7953151515152 7.36485491235823e-05
% -56.4928303030303 7.36485491235823e-05
% -55.1903454545455 7.36485491235823e-05
% -53.8878606060606 0.000147297098247165
% -52.5853757575758 0.000147297098247165
% -51.2828909090909 0.000147297098247165
% -49.9804060606061 0.000294594196494329
% -48.6779212121212 0.000294594196494329
% -47.3754363636364 0.000294594196494329
% -46.0729515151515 0.000368242745617911
% -44.7704666666667 0.000368242745617911
% -43.4679818181818 0.000515539843865076
% -42.165496969697 0.000736485491235823
% -40.8630121212121 0.000736485491235823
% -39.5605272727273 0.000810134040359405
% -38.2580424242424 0.00103107968773015
% -36.9555575757576 0.0012520253351009
% -35.6530727272727 0.00132567388422448
% -34.3505878787879 0.00162026808071881
% -33.048103030303 0.00213580792458389
% -31.7456181818182 0.00265134776844896
% -30.4431333333333 0.00338783325968478
% -29.1406484848485 0.00390337310354986
% -27.8381636363636 0.00441891294741494
% -26.5356787878788 0.00530269553689792
% -25.2331939393939 0.00640742377375166
% -23.9307090909091 0.00714390926498748
% -22.6282242424242 0.00824863750184121
% -21.3257393939394 0.00972160848431286
% -20.0232545454545 0.0108999852702902
% -18.7207696969697 0.0126675504492561
% -17.4182848484849 0.0148770069229636
% -16.1158 0.0173074090440418
% -14.8133151515152 0.0190013256738842
% -13.5108303030303 0.0224628074826926
% -12.2083454545455 0.0265871262336132
% -10.9058606060606 0.0310060391810281
% -9.60337575757576 0.0357195463249374
% -8.30089090909092 0.0425688613934306
% -6.99840606060607 0.0517012814847548
% -5.69592121212121 0.0601708646339667
% -4.39343636363637 0.0704816615112682
% -3.09095151515152 0.0813816467815584
% -1.78846666666667 0.0936073059360731
% -0.48598181818182 0.105317425246723
% 0.816503030303025 0.116806598910001
% 2.11898787878787 0.130431580497864
% 3.42147272727272 0.143614670790985
% 4.72395757575757 0.157755192222713
% 6.02644242424243 0.171527470908823
% 7.32892727272726 0.183458535866843
% 8.63141212121212 0.196936220356459
% 9.93389696969697 0.20908823096185
% 11.2363818181818 0.219914567683017
% 12.5388666666667 0.230519958756812
% 13.8413515151515 0.242377375165709
% 15.1438363636364 0.254971277065842
% 16.4463212121212 0.277875975843276
% 17.7488060606061 0.30880836647518
% 19.0512909090909 0.339151568714096
% 20.3537757575758 0.368316394167035
% 21.6562606060606 0.397260273972603
% 22.9587454545454 0.429739284136103
% 24.2612303030303 0.465679776108411
% 25.5637151515151 0.500736485491236
% 26.8662 0.556930328472529
% 28.1686848484848 0.631020768890853
% 29.4711696969697 0.694432169686257
% 30.7736545454545 0.745912505523641
% 32.0761393939394 0.79091176903815
% 33.3786242424242 0.829429960229783
% 34.6811090909091 0.855354249521284
% 35.9835939393939 0.868316394167035
% 37.2860787878788 0.876270437472382
% 38.5885636363636 0.883046103991751
% 39.8910484848485 0.890190013256739
% 41.1935333333333 0.897849462365591
% 42.4960181818182 0.901900132567388
% 43.798503030303 0.904551480335837
% 45.1009878787879 0.907129179555163
% 46.4034727272727 0.908675799086758
% 47.7059575757576 0.912137280895566
% 49.0084424242424 0.921269700986891
% 50.3109272727273 0.930254823979968
% 51.6134121212121 0.935778465164236
% 52.915896969697 0.940565620857269
% 54.2183818181818 0.943437914273089
% 55.5208666666667 0.946899396081897
% 56.8233515151515 0.95168655177493
% 58.1258363636364 0.960450729120636
% 59.4283212121212 0.969288555015466
% 60.730806060606 0.974664899101488
% 62.0332909090909 0.97738989541906
% 63.3357757575757 0.979378406245397
% 64.6382606060606 0.980630431580498
% 65.9407454545454 0.983870967741935
% 67.2432303030303 0.985859478568272
% 68.5457151515151 0.992414199440271
% 69.8482 1
% };

\addplot [semithick, color2]
table {%
-70.7047 7.36485491235823e-05
-69.2514686868687 7.36485491235823e-05
-67.7982373737374 7.36485491235823e-05
-66.3450060606061 0.000147297098247165
-64.8917747474748 0.000147297098247165
-63.4385434343434 0.000147297098247165
-61.9853121212121 0.000147297098247165
-60.5320808080808 0.000147297098247165
-59.0788494949495 0.000147297098247165
-57.6256181818182 0.000147297098247165
-56.1723868686869 0.000147297098247165
-54.7191555555556 0.000147297098247165
-53.2659242424242 0.000220945647370747
-51.8126929292929 0.000220945647370747
-50.3594616161616 0.000368242745617911
-48.9062303030303 0.000368242745617911
-47.452998989899 0.000441891294741494
-45.9997676767677 0.000441891294741494
-44.5465363636364 0.000515539843865076
-43.0933050505051 0.00066283694211224
-41.6400737373737 0.000736485491235823
-40.1868424242424 0.000957431138606569
-38.7336111111111 0.00117837678597732
-37.2803797979798 0.00154661953159523
-35.8271484848485 0.00162026808071881
-34.3739171717172 0.00228310502283105
-32.9206858585859 0.00265134776844896
-31.4674545454546 0.00294594196494329
-30.0142232323232 0.00368242745617911
-28.5609919191919 0.00434526439829135
-27.1077606060606 0.00544999263514509
-25.6545292929293 0.00692296361761673
-24.201297979798 0.00802769185447047
-22.7480666666667 0.00927971718957137
-21.2948353535354 0.010752688172043
-19.841604040404 0.0133303873913684
-18.3883727272727 0.0150979525703344
-16.9351414141414 0.0171601119457947
-15.4819101010101 0.0203269995581087
-14.0286787878788 0.0233465900721756
-12.5754474747475 0.0268080718809839
-11.1222161616162 0.0311533362792753
-9.66898484848485 0.0378553542495213
-8.21575353535354 0.0443364265723965
-6.76252222222223 0.0540580350567094
-5.30929090909092 0.0629695095006628
-3.85605959595961 0.0749742230078067
-2.4028282828283 0.0853586684342318
-0.949596969696984 0.0982471645308587
0.503634343434342 0.111577551922227
1.95686565656565 0.124907939313596
3.41009696969697 0.137870083959346
4.86332828282828 0.150537634408602
6.31655959595959 0.164899101487701
7.7697909090909 0.177934894682575
9.22302222222221 0.191265282073943
10.6762535353535 0.203932832523199
12.1294848484848 0.215790248932096
13.5827161616161 0.227647665340993
15.0359474747475 0.243850346148181
16.4891787878788 0.276918544704669
17.9424101010101 0.311165120047135
19.3956414141414 0.343275887465017
20.8488727272727 0.375754897628517
22.302104040404 0.406613639711298
23.7553353535353 0.440344675209898
25.2085666666667 0.479157460598026
26.661797979798 0.542126970098689
28.1150292929293 0.623066725585506
29.5682606060606 0.68647812638091
31.0214919191919 0.736706436883193
32.4747232323232 0.784283399617028
33.9279545454545 0.82051848578583
35.3811858585859 0.84312859036677
36.8344171717172 0.861098836352924
38.2876484848485 0.874060980998674
39.7408797979798 0.884077183679482
41.1941111111111 0.89041095890411
42.6473424242424 0.896008248637502
44.1005737373737 0.90050081013404
45.553805050505 0.906319045514803
47.0070363636364 0.913168360583297
48.4602676767677 0.921196052437767
49.913498989899 0.931285903667698
51.3667303030303 0.937472381794079
52.8199616161616 0.940933863602887
54.2731929292929 0.944321696862572
55.7264242424242 0.948225069966122
57.1796555555555 0.953896008248638
58.6328868686869 0.963470319634703
60.0861181818182 0.972013551333039
61.5393494949495 0.976800707026072
62.9925808080808 0.977758138164678
64.4458121212121 0.978789217852408
65.8990434343434 0.980777728678745
67.3522747474747 0.982692590955958
68.805506060606 0.983576373545441
70.2587373737374 0.987111503903373
71.7119686868687 0.995507438503461
73.1652 1
};
\end{axis}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{SINR DL enb=8x8_ue=4x4_bfType=ns3::MmWaveCodebookBeamforming_cbUpdatePeriod=100};
\end{tikzpicture}


==> figures/fs/thr_dl_enb8x8_ue4x4_enbAntennaTypeThreeGppAntennaModel.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={IPI [us]},
ylabel={Throughput [bps]},
xmajorgrids,
xmin=0.5, xmax=2.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-114812312.707002, ymax=2411058566.84704,
ytick style={color=black},
xtick={1, 2},
xticklabels={10, 1000},
ybar,
ymode=log
]
\addplot [semithick, color0]
table {%
1 2208238954.73534
% 100 0
2 23828059.8073776
};
\addplot [semithick, color1]
table {%
1 2296246254.14003
% 100 0
2 23831396.0377673
};
% \addplot [semithick, color2]
% table {%
% 10 0
% 100 0
% 1000 23755365.1030972
% };
% \addplot [semithick, color3]
% table {%
% 10 0
% 100 0
% 1000 23821562.9376714
% };
% \addplot [semithick, color4]
% table {%
% 10 1948105696.42702
% 100 0
% 1000 23728499.6689067
% };
% \addplot [semithick, color5]
% table {%
% 10 2003496076.04041
% 100 0
% 1000 23735874.4939786
% };
% \addplot [semithick, color6]
% table {%
% 10 0
% 100 0
% 1000 22938515.4308454
% };
% \addplot [semithick, white!49.8039215686275!black]
% table {%
% 10 0
% 100 0
% 1000 22766787.3613135
% };
\end{axis}

% \draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
%   scale=0.6,
%   anchor=north,
%   text=black,
%   rotate=0.0
% ]{THR DL enb=8x8_ue=4x4_enbAntennaType=ns3::ThreeGppAntennaModel};
\end{tikzpicture}


==> figures/fs/thr_dl_enb8x8_ue4x4_enbAntennaTypeThreeGppAntennaModel_2.tex <==
\definecolor{my-blue-bar}{RGB}{114,147,203}
\definecolor{my-red-bar}{RGB}{211,94,96}

\pgfplotsset{scaled y ticks=false}
\pgfplotsset{
% override style for non-boxed plots
    % which is the case for both sub-plots
    every non boxed x axis/.style={}
}
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=my fancy plots,
        group size=1 by 2,
        xticklabels at=edge bottom,
        vertical sep=0pt
    },
    width=8.5cm,
    xmin=-6, xmax=6
]

\nextgroupplot[ymin=1.5e9,ymax=2400000000,
							 xmin=-0.2, xmax=1.475,
               ytick={2e9},
               yticklabels={$2*10^9$},
               axis x line=top,
               xtick={0.1375,1.1375},
               axis y discontinuity=parallel,
               height=3.0cm,
							 y grid style={white!69.01960784313725!black},
							 ymajorgrids,
							 ticklabel style = {font=\footnotesize},
							 % legend style={font=\footnotesize}
               ]

							 \draw[fill=my-red-bar,draw opacity=0] (axis cs:0.15,1.7e8) rectangle (axis cs:0.35,2208238954.73534);
               \draw[fill=my-blue-bar,draw opacity=0] (axis cs:-0.075,1.7e8) rectangle (axis cs:0.125,2296246254.14003);
               \draw[fill=white,draw opacity=0] (axis cs:-0.075,1.6e9) rectangle (axis cs:0.35,1.68e9);
               \draw[] (-0.085,1.6e9) -- (0.135,1.6e9);
               \draw[] (-0.085,1.68e9) -- (0.135,1.68e9);
               \draw[] (0.14,1.6e9) -- (0.36,1.6e9);
               \draw[] (0.14,1.68e9) -- (0.36,1.68e9);
						   \addlegendimage{ybar,ybar legend,fill=my-red-bar,draw opacity=0, font=\footnotesize};
						   \addlegendentry{SVD}

						   %\draw[fill=my-blue-bar,draw opacity=0] (axis cs:1.15,423) rectangle (axis cs:1.35,0);
						   \addlegendimage{ybar,ybar legend,fill=my-blue-bar,draw opacity=0, font=\footnotesize};
						   \addlegendentry{Codebook}

						   %\addplot [semithick, black, forget plot]
						   %table[row sep=crcr] {%
						   %-0.22475 419.7\\
						   %-0.17525 420.3\\
						   %};
						   %\addplot [semithick, black, forget plot]
						   %table[row sep=crcr] {%
						   %1.42525 419.7\\
						   %1.47475 420.3\\
						   %};

\nextgroupplot[ymin=0,ymax=3.5e7,
               ytick={0, 1e7, 2e7, 3e7},
               yticklabels={0, $1*10^7$, $2*10^7$, $3*10^7$},
							 xmin=-0.2, xmax=1.475,
							 ylabel={Throughput [bps]},
							 ylabel style={font=\footnotesize\color{white!15!black}, at={(ticklabel cs:0.7)}},
               %ytick={0},
               axis x line=bottom,
							 xtick={0.1375,1.1375},
							 xticklabels={10, 1000},
               height=4.5cm,
							 y grid style={white!69.01960784313725!black},
							 ymajorgrids,
							 ticklabel style = {font=\footnotesize}]

							 \draw[fill=my-blue-bar,draw opacity=0] (axis cs:-0.075,0) rectangle (axis cs:0.125,2.5e8);
							 \draw[fill=my-blue-bar,draw opacity=0] (axis cs:0.925,0) rectangle (axis cs:1.125,23828059.8073776);
							 \draw[fill=my-red-bar,draw opacity=0] (axis cs:0.15,0) rectangle (axis cs:0.35,2.5e8);
							 \draw[fill=my-red-bar,draw opacity=0] (axis cs:1.15,0) rectangle (axis cs:1.35,23831396.0377673);
							 %\addplot [semithick, black]
							 %table[row sep=crcr] {%
							 %-0.22475 1.97\\
							 %-0.17525 2.03\\
							 %};
							 %\addplot [semithick, black]
							 %table[row sep=crcr] {%
							 %1.42525 1.97\\
							 %1.47475 2.03\\
							 %};
\end{groupplot}

\end{tikzpicture}


==> figures/fs/thr_dl_ut_1enb8x8_ue4x4_enbAntennaTypeThreeGppAntennaModel.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={IPI [us]},
xmajorgrids,
xmin=-39.5, xmax=1049.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-55233629.4615895, ymax=1159906218.69338,
ytick style={color=black},
ytick={-200000000,0,200000000,400000000,600000000,800000000,1000000000,1200000000},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2}
]
\addplot [semithick, color0]
table {%
10 1022938632.0984
100 0
1000 11912273.9927819
};
\addplot [semithick, color1]
table {%
10 1104672589.23179
100 0
1000 11915610.2231715
};
\addplot [semithick, color2]
table {%
10 0
100 0
1000 11839579.2885026
};
\addplot [semithick, color3]
table {%
10 0
100 0
1000 11905777.1230758
};
\addplot [semithick, color4]
table {%
10 865308594.240259
100 0
1000 11812713.8543124
};
\addplot [semithick, color5]
table {%
10 816955553.65692
100 0
1000 11820088.6793843
};
\addplot [semithick, color6]
table {%
10 0
100 0
1000 11127206.3047801
};
\addplot [semithick, white!49.8039215686275!black]
table {%
10 0
100 0
1000 10917726.154526
};
\end{axis}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{THR DL UT 1enb=8x8_ue=4x4_enbAntennaType=ns3::ThreeGppAntennaModel};
\end{tikzpicture}


==> figures/fs/thr_dl_ut_2enb8x8_ue4x4_enbAntennaTypesThreeGppAntennaModel.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={IPI [us]},
xmajorgrids,
xmin=-39.5, xmax=1049.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-59578683.243721, ymax=1251152348.11814,
ytick style={color=black},
ytick={-200000000,0,200000000,400000000,600000000,800000000,1000000000,1200000000,1400000000},
yticklabels={−0.2,0.0,0.2,0.4,0.6,0.8,1.0,1.2,1.4}
]
\addplot [semithick, color0]
table {%
10 1185300322.6044
100 0
1000 11915785.8142447
};
\addplot [semithick, color1]
table {%
10 1191573664.87442
100 0
1000 11915785.8142447
};
\addplot [semithick, color2]
table {%
10 0
100 0
1000 11915785.8142447
};
\addplot [semithick, color3]
table {%
10 0
100 0
1000 11915785.8142447
};
\addplot [semithick, color4]
table {%
10 1082797102.15806
100 0
1000 11915785.8142447
};
\addplot [semithick, color5]
table {%
10 1186540522.35398
100 0
1000 11915785.8142447
};
\addplot [semithick, color6]
table {%
10 0
100 0
1000 11811309.1257273
};
\addplot [semithick, white!49.8039215686275!black]
table {%
10 0
100 0
1000 11849061.2064521
};
\end{axis}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=north,
  text=black,
  rotate=0.0
]{THR DL UT 2enb=8x8_ue=4x4_enbAntennaType=ns3::ThreeGppAntennaModel};
\end{tikzpicture}

